Efficient Adaptation of Pre-trained Vision Transformer underpinned by Approximately Orthogonal Fine-Tuning Strategy

A prevalent approach in Parameter-Efficient Fine-Tuning (PEFT) of pre-trained Vision Transformers (ViT) involves freezing the majority of the backbone parameters and solely learning low-rank adaptation weight matrices to accommodate downstream tasks. These low-rank matrices are commonly derived through the multiplication structure of down-projection and up-projection matrices, exemplified by methods such as LoRA and Adapter. In this work, we observe an approximate orthogonality among any two row or column vectors within any weight matrix of the backbone parameters; however, this property is absent in the vectors of the down/up-projection matrices. Approximate orthogonality implies a reduction in the upper bound of the model's generalization error, signifying that the model possesses enhanced generalization capability. If the fine-tuned down/up-projection matrices were to exhibit this same property as the pre-trained backbone matrices, could the generalization capability of fine-tuned ViTs be further augmented? To address this question, we propose an Approximately Orthogonal Fine-Tuning (AOFT) strategy for representing the low-rank weight matrices. This strategy employs a single learnable vector to generate a set of approximately orthogonal vectors, which form the down/up-projection matrices, thereby aligning the properties of these matrices with those of the backbone. Extensive experimental results demonstrate that our method achieves competitive performance across a range of downstream image classification tasks, confirming the efficacy of the enhanced generalization capability embedded in the down/up-projection matrices.

==> sec/sup.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_init/query_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of initialized matrices $\mathbf{W}_{q}$.}
        \label{fig:vit-query-init}
    \end{subfigure}
    %\hfill % 添加水平填充以分隔子图
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_init/key_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of initialized matrices $\mathbf{W}_{k}$.}
        \label{fig:vit-key-init}
    \end{subfigure}
    %\hfill % 添加水平填充以分隔子图
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_init/value_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of initialized matrices $\mathbf{W}_{v}$.}
        \label{fig:vit-value-init}
    \end{subfigure}
    %\hfill % 添加水平填充以分隔子图
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_init/out_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of initialized matrices $\mathbf{W}_{o}$.}
        \label{fig:vit-out-init}
    \end{subfigure}
    %\hfill % 添加水平填充以分隔子图
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_init/fc1_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of initialized matrices $\mathbf{W}_{\rm FC1}$.}
        \label{fig:vit-fc1-init}
    \end{subfigure}
    %\hfill % 添加水平填充以分隔子图
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_init/fc2_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of initialized matrices $\mathbf{W}_{\rm FC2}$.}
        \label{fig:vit-fc2-init}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_pre/query_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of pre-trained matrices $\mathbf{W}_{q}$.}
        \label{fig:vit-query-pre-train}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_pre/key_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of pre-trained matrices $\mathbf{W}_{k}$.}
        \label{fig:vit-key-pre-train}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_pre/value_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of pre-trained matrices $\mathbf{W}_{v}$.}
        \label{fig:vit-value-pre-train}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_pre/out_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of pre-trained matrices $\mathbf{W}_{o}$.}
        \label{fig:vit-out-pre-train}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_pre/fc1_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of pre-trained matrices $\mathbf{W}_{\mathrm {FC1}}$.}
        \label{fig:vit-fc1-pre-train}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{figure/Vit_pre/fc2_angle_distribution.pdf} % 替换为你的图片路径
        \caption{The degree distribution of pre-trained matrices $\mathbf{W}_{\mathrm {FC2}}$.}
        \label{fig:vit-fc2-pre-train}
    \end{subfigure}
    \caption{Illustration of approximate orthogonality among any two column vectors of weight matrices $\mathbf{W}_{q}, \mathbf{W}_{k}, \mathbf{W}_{v}, \mathbf{W}_{o}, \mathbf{W}_\mathrm{FC1}, \mathbf{W}_\mathrm{FC2}$ in the ViT-B model after training. The histogram represents the distribution of angles between any two column vectors within each weight matrix. Specifically, \subref{fig:vit-query-init}-\subref{fig:vit-fc2-init} represent approximate orthogonality at the initialization stage, while \subref{fig:vit-query-pre-train}-\subref{fig:vit-fc2-pre-train} represent approximate orthogonality in the pre-trained model.}
    \label{fig:vit-init-pre-train}
\end{figure*}

